Query strategy for sequential ontology debugging

Debugging of ontologies is an important prerequisite for their wide-spread application, especially in areas that rely upon everyday users to create and maintain knowledge bases, as in the case of the Semantic Web. Recent approaches use diagnosis methods to identify causes of inconsistent or incoherent ontologies. However, in most debugging scenarios these methods return many alternative diagnoses, thus placing the burden of fault localization on the user. This paper demonstrates how the target diagnosis can be identified by performing a sequence of observations, that is, by querying an oracle about entailments of the target ontology. We exploit a-priori probabilities of typical user errors to formulate information-theoretic concepts for query selection. Our evaluation showed that the proposed method significantly reduces the number of required queries compared to myopic strategies. We experimented with different probability distributions of user errors and different qualities of the a-priori probabilities. Our measurements showed the advantageousness of information-theoretic approach to query selection even in cases where only a rough estimate of the priors is available.

==> 1.introduction.tex <==
\section{Introduction}
Acquisition and maintenance of knowledge bases is an important prerequisite for a successful application of semantic systems in areas such as the Semantic Web. At the current state of the art ontology extraction methods do not allow a complete and error free automatic acquisition of ontologies. Thus users of semantic systems are required to formulate and correct logical descriptions on their own. In most of the cases these users are domain experts who have little or no experience in expressing their knowledge in representation languages like OWL~\cite{Grau2008a}. 
%
Studies in cognitive psychology, e.g.~\cite{Ceraso71,Johnson1999}, discovered that humans make systematic errors while formulating or interpreting logical descriptions. Results presented in~\cite{Rector2004,Roussey2009} confirmed these observations regarding ontology development. Therefore it is essential to create methods that can identify and correct erroneous ontological definitions. 

Ontology debugging methods~\cite{schlobach2007,Kalyanpur.Just.ISWC07,friedrich2005gdm,Horridge2008} simplify the development of ontologies. 
% MOD to the end of par
Usually the main requirement for the debugging process is to obtain a consistent and, optionally, coherent ontology. 
These basic requirements can be extended by additional ones, 
such as test cases~\cite{friedrich2005gdm}, which must be fulfilled by the target ontology $\mo_t$.
Given the requirements (e.g.\ formulated by a user) an ontology debugger identifies a set of alternative diagnoses, where each diagnosis corresponds to a set of possibly faulty axioms.  In particular, a \emph{diagnosis} $\md$ is a subset of an ontology $\mo$ such that removal of the diagnosis from the ontology (i.e.\ $\mo \setminus \md$) will allow the formulation of the target ontology $\mo_t$ that fulfills all the requirements. We call the removal of a diagnosis from the ontology a \emph{trivial application} of a diagnosis.
Moreover, in practical applications it might be inefficient to consider all possible diagnoses. Therefore, modern ontology debugging approaches focus on the computation of minimal diagnoses, i.e.\ such diagnoses $\md_i$ that no $\md'_i \subset \md_i$ is a diagnosis. A user has to change at least all of the axioms of a minimal diagnosis in order to formulate the intended target ontology. 
% END

However, the diagnosis methods can return many alternative minimal diagnoses for a given set of test cases and requirements. 
% MOD
A sample study of real-world incoherent ontologies, which were used in~\cite{Kalyanpur.Just.ISWC07}, shows that there may exist hundreds or even thousands of minimal diagnoses. 
% END
In the case of the Transportation ontology the diagnosis method was able to identify 1782 minimal diagnoses~\footnote{Subsequently, we will give a detailed characterization of these ontologies.}. In such situations some simple visualization of all alternative modifications of the ontology is ineffective. The goal of sequential debugging is to identify the set of axioms $\md_t$ of an ontology which have to be changed or removed in order to formulate the target ontology $\mo_t$. The set of axioms $\md_t$ is called the target diagnosis. 
% MOD
Consequently, the target ontology corresponds to the ontology resulting from a removal of the target diagnosis from the original ontology and an extension by some additional axioms $EX$, i.e.\ $\mo_t = (\mo \setminus \md_t) \cup EX$.
% END


%Note, even a small number of \emph{minimal conflicts} can be a source of a large number of diagnoses.
A possible solution of the problem would be to introduce an order on the set of diagnoses by means of some preference criteria. For instance, Kalyanpur et al.~\cite{Kalyanpur2006} suggest measures to rank the axioms of a diagnosis depending on their structure, occurrence in test cases, etc. Only the top ranking diagnoses are then presented to the user.
Of course this set of diagnoses will contain the target diagnosis only in the case when a faulty ontology, the given requirements and test cases, provide sufficient data to the appropriate heuristic. Therefore, in most debugging sessions a user has to input additional information (e.g.\ tests in form of required implications of facts or axioms) to identify the target diagnosis. However, it is hard to guess, which information is required. That is, a user does not know a priori which and how many tests should be provided to the debugger, such that it will return the target diagnosis. 

In this paper we present an approach for the acquisition of additional information by generating a sequence of queries, which should be answered by some oracle such as a user, an information extraction system, etc. Each answer to a query is used by our method to reduce the set of diagnoses until, finally, the target diagnosis is identified. In order to construct queries we exploit the property that different  ontologies resulting from trivial applications of different diagnoses entail unequal sets of axioms. 
Consequently, we can differentiate between diagnoses by asking the oracle if the target ontology should imply a logical sentence or not. These implied logical sentences can be generated by classification and realization services provided in description logic reasoning systems~\cite{Sirin2007Pellet,Haarslev2001,Motik2009}. In particular, the classification process computes a subsumption hierarchy (sometimes also called ``inheritance hierarchy'' of parents and children) for each concept name mentioned in a TBox. For each individual mentioned in an ABox, the realization computes the atomic classes (or concept names) of which the individual is an instance~\cite{Sirin2007Pellet}. 

In order to generate the most informative query we exploit the fact that some diagnoses are more likely than others because of typical user errors~\cite{Rector2004,Roussey2009}. User's beliefs for an error to occur in some part of a knowledge base, represented as  probabilities, can be used to estimate the change in entropy of the set of diagnoses if a particular query is answered. 
We select those queries which minimize the expected entropy, i.e.\ maximize the information gain. An oracle should answer these queries until a diagnosis is identified whose probability is significantly higher than those of all other diagnoses. This diagnosis is the most likely to be the target one. 

We compare our entropy-based method with a greedy approach that selects those queries which try to cut the number of diagnoses in half. The evaluation is performed using generated examples as well as real-world ontologies presented in Table~\ref{tab:motivation}. In the first case we alter a consistent and coherent ontology with additional axioms to generate such conflicts that result in a predefined number of diagnoses of required length. A faulty ontology is then analyzed by the debugging algorithm using entropy, greedy and ``random'' strategies, where the latter selects queries to be asked completely randomly. Evaluation results show that on average the suggested entropy-based approach is almost $50\%$ better than the greedy one. In the second evaluation scenario we analyzed the performance of entropy-based and greedy strategies on real-world ontologies given different input settings. In particular, we simulated different strategies for a user to assign prior probabilities as well as the quality of these probabilities that might occur in practice. The obtained results show that the entropy method outperformed the greedy heuristic in most of the cases. In some situations the entropy-based approach  achieved twice as good average performance compared to the greedy one. Moreover, the evaluation on the real-world ontologies showed that the entropy-based query selection is robust to the actual values of prior fault probabilities as well as differences between them. It is only important whether the specified priors favor the target diagnosis or not.   

The remainder of the paper is organized as follows: Section~\ref{sect:example} presents two introductory examples as well as the basic concepts. The details of the entropy-based query selection method are given in Section~\ref{sect:theory}. Section~\ref{sect:impl} describes the implementation of the approach and is followed by evaluation results in Section~\ref{sect:eval}. The paper concludes with an overview on related work.

